VLBI Probes of Jet Physics in Neutrino-Candidate Blazars

In recent years, evidence has accumulated that some high-energy cosmic neutrinos can be associated with blazars. The strongest evidence for an individual association was found in the case of the blazar TXS 0506+056 in 2017. In July 2019, another track-like neutrino event (IC190730A) was found spatially coincident with the well-known bright flat-spectrum radio quasar PKS 1502+106. PKS 1502+106 was not found to be in a particularly elevated gamma-ray state, but exhibited a remarkably bright radio outburst at the time of the neutrino detection, similar to TXS 0506+056. We have performed a multi-frequency VLBI study from 15 GHz up to 86 GHz on TXS 0506+056, PKS 1502+106 and one additional neutrino-candidate blazar (PKS 0215+015) to study the radio structure of neutrino candidate blazars in response to their neutrino association. We have obtained target of opportunity observations with the VLBA for all three sources within $\sim$1 month from their associated neutrino events and are performing multi-epoch studies of the jet kinematics at 15 GHz as part of the MOJAVE program. Here, we present first results on TXS 0506+056 at 86 GHz and one additional 43 GHz image obtained 27 days after IC170922A, closer in time to the neutrino event than previously published images. We also give an overview about our recent work on PKS 1502+106 and PKS 0215+015.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

